Probabilistic Tube-based Control Synthesis of Stochastic Multi-Agent Systems under Signal Temporal Logic

We consider the control design of stochastic discrete-time linear multi-agent systems (MASs) under a global signal temporal logic (STL) specification to be satisfied at a predefined probability. By decomposing the dynamics into deterministic and error components, we construct a probabilistic reachable tube (PRT) as the Cartesian product of reachable sets of the individual error systems driven by disturbances lying in confidence regions (CRs) with a fixed probability. By bounding the PRT probability with the specification probability, we tighten all state constraints induced by the STL specification by solving tractable optimization problems over segments of the PRT, and relax the underlying stochastic problem with a deterministic one. This approach reduces conservatism compared to tightening guided by the STL structure. Additionally, we propose a recursively feasible algorithm to attack the resulting problem by decomposing it into agent-level subproblems, which are solved iteratively according to a scheduling policy. We demonstrate our method on a ten-agent system, where existing approaches are impractical.

==> compute_times_comparison.tex <==
\begin{tikzpicture}
    \begin{axis}[
        xlabel={Number of Agents},
        ylabel={Runtime (s)},
        xtick={1,2,3,4,5,6,7,8,9,10},
        ymode=log, % Use logarithmic scale for the y-axis
        log basis y={10}, % Base 10 logarithm
        legend pos=north west,
        grid=both,
        grid style={line width=.1pt, draw=gray!10},
        major grid style={line width=.2pt,draw=gray!50},
        %minor y tick num=5,
        width=3.45in,
        height=1.6in
    ]
    
    % Algorithm 1 data points
    \addplot[
        color=blue,
        mark=square*,
        thick
    ] coordinates {
        (1, 4.8)
        (2, 12.08)
        (3, 22.32)
        (4, 36.88)
        (5, 39.18)
        (6, 45.67)
        (7, 58.73)
        (8, 98.35)
        (9, 143.51)
        (10, 321.81)
    };
    \addlegendentry{Algorithm 1}
    
    % Centralized data points
    \addplot[
        color=red,
        mark=*,
        thick
    ] coordinates {
        (1, 4.8)
        (2, 57.07)
        (3, 93.6972)
        (4, 173.91)
        (5, 491.3345)
        (6, 810.1268)
        (7, 2.0811e+03)
        (8, 3.2577e+03)
        (9, 4.3629e+03)
        (10, 9832.15)
    };
    \addlegendentry{Centralized}

    \end{axis}
\end{tikzpicture}
